Electromechanical phenomena in normal and superconducting nanostructures based on a movable quantum dot

The dissertation is devoted to the study of new fundamental phenomena which emerge due to electromechanical coupling in mesoscopic systems based on movable quantum dot.

==> Dissertation/Makefile <==
all:
	latexmk -pdf -pdflatex="xelatex %O %S" dissertation
pdf:
	latexmk -pdf -jobname=synopsis_pdf -silent  dissertation.tex
draft:	
	pdflatex -ini -jobname="draft-preamble" "&pdflatex draft-preamble.tex\dump"
	latexmk -pdf -jobname=draft -silent --shell-escape draft.tex

clean:
	latexmk -C dissertation
	rm -f dissertation.bbl

distclean:
	## Core latex/pdflatex auxiliary files:
	rm -f *.aux
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.fls
	rm -f *.out
	rm -f *.toc

	## Intermediate documents:
	rm -f *.dvi
	rm -f *-converted-to.*
	# these rules might exclude image files for figures etc.
	# *.ps
	# *.eps
	# *.pdf

	## Bibliography auxiliary files (bibtex/biblatex/biber):
	rm -f *.bbl
	rm -f *.bcf
	rm -f *.blg
	rm -f *-blx.aux
	rm -f *-blx.bib
	rm -f *.brf
	rm -f *.run.xml

	## Build tool auxiliary files:
	rm -f *.fdb_latexmk
	rm -f *.synctex
	rm -f *.synctex.gz
	rm -f *.synctex.gz\(busy\)
	rm -f *.pdfsync

	## Auxiliary and intermediate files from other packages:

	# algorithms
	rm -f *.alg
	rm -f *.loa

	# achemso
	rm -f acs-*.bib

	# amsthm
	rm -f *.thm

	# beamer
	rm -f *.nav
	rm -f *.snm
	rm -f *.vrb

	#(e)ledmac/(e)ledpar
	rm -f *.end
	rm -f *.[1-9]
	rm -f *.[1-9][0-9]
	rm -f *.[1-9][0-9][0-9]
	rm -f *.[1-9]R
	rm -f *.[1-9][0-9]R
	rm -f *.[1-9][0-9][0-9]R
	rm -f *.eledsec[1-9]
	rm -f *.eledsec[1-9]R
	rm -f *.eledsec[1-9][0-9]
	rm -f *.eledsec[1-9][0-9]R
	rm -f *.eledsec[1-9][0-9][0-9]
	rm -f *.eledsec[1-9][0-9][0-9]R

	# glossaries
	rm -f *.acn
	rm -f *.acr
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls

	# gnuplottex
	rm -f *-gnuplottex-*

	# hyperref
	rm -f *.brf

	# knitr
	rm -f *-concordance.tex
	rm -f *.tikz
	rm -f *-tikzDictionary

	# listings
	rm -f *.lol

	# makeidx
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist

	# minitoc
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc[0-9]
	rm -f *.mtc[1-9][0-9]

	# minted
	rm -f _minted*
	rm -f *.pyg

	# morewrites
	rm -f *.mw

	# mylatexformat
	rm -f *.fmt

	# nomencl
	rm -f *.nlo

	# sagetex
	rm -f *.sagetex.sage
	rm -f *.sagetex.py
	rm -f *.sagetex.scmd

	# sympy
	rm -f *.sout
	rm -f *.sympy
	rm -f sympy-plots-for-*.tex/

	# pdfcomment
	rm -f *.upa
	rm -f *.upb

	#pythontex
	rm -f *.pytxcode
	rm -f pythontex-files-*/

	# Texpad
	rm -f .texpadtmp

	# TikZ & PGF
	rm -f *.dpth
	rm -f *.md5
	rm -f *.auxlock

	# todonotes
	rm -f *.tdo

	# xindy
	rm -f *.xdy

	# WinEdt
	rm -f *.bak
	rm -f *.sav

	# endfloat
	rm -f *.ttt
	rm -f *.fff
	rm -f *.aux
	rm -f *.bbl
	rm -f *.blg
	rm -f *.dvi
	rm -f *.fdb_latexmk
	rm -f *.fls
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.nav
	rm -f *.nlo
	rm -f *.out
	rm -f *.pdfsync
	rm -f *.ps
	rm -f *.snm
	rm -f *.synctex.gz
	rm -f *.toc
	rm -f *.vrb
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc0
	rm -f *.bak
	rm -f *.bcf
	rm -f *.run.xml


==> Dissertation/lists.tex <==
\clearpage
\phantomsection
\addcontentsline{toc}{chapter}{\listfigurename}
\listoffigures									% Список изображений


%%% Список таблиц %%%
% (ГОСТ Р 7.0.11-2011, 5.3.10)
\clearpage
\phantomsection
\addcontentsline{toc}{chapter}{\listtablename}
\listoftables									% Список таблиц
\newpage

==> Dissertation/title.tex <==

\thispagestyle{empty}%
\begin{center}%
\MakeUppercase{\textbf{Національна академія наук України \\ Фізико-технічний інститут низьких температур }}\\ \textbf{імені Б.І.~Вєркіна}
\end{center}%
%

\begin{center}%
\MakeUppercase{Національна академія наук України \\ Фізико-технічний інститут низьких температур}\\ імені Б.І.~Вєркіна
\end{center}%
%

\begin{flushright}%
Кваліфікаційна наукова \\ праця на правах рукопису


%
\vspace{0pt plus6fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}%
{\textbf{\thesisAuthor} }
\end{center}%
%
\text {УДК 538.93}
\end{flushright}%
%
\begin{center}%
\textbf{ДИСЕРТАЦІЯ}
\end{center}%
%
\vspace{0pt plus1fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}%
\textbf {\large \MakeUppercase{Електромеханічні явища\\ в нормальних та надпровідних наноструктурах\\ на основі рухомої квантової точки}}

\vspace{0pt plus2fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
{%\small
104 --- <<Фізика та астрономія>>\\ 
10~--- <<Природничі науки>>
}

\vspace{0pt plus2fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
Подається на здобуття наукового ступеня доктора філософії 


%
\vspace{0pt plus4fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
%
{\small Дисертація містить результати власних досліджень. Використання ідей, результатів і текстів інших авторів мають посилання на відповідне джерело $\underset{\text{(підпис здобувача)}}{\underline{\hspace{0.16\textwidth}}}$ O.M.~Багрова}
%
\end{center}%
%
\vspace{0pt plus4fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{flushright}%
\textbf{Науковий керівник:~Кулініч Сергій Іванович,\\ кандидат фізико-математичних наук,\\ старший науковий співробітник}
\end{flushright}%
%
%{\small Всі примірники дисертації ідентичні за змістом. \\
%Учений секретар... }
%
\vspace{0pt plus4fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}%
{\thesisCity~--~2023}
\end{center}%
\newpage


==> Makefile <==
all: synopsis dissertation

dissertation:
	#	$(MAKE) -C Dissertation
	latexmk -pdf -pdflatex="xelatex %O %S" dissertation

synopsis:
	#	$(MAKE) -C Synopsis
	latexmk -pdf -pdflatex="xelatex %O %S" synopsis

draft:
	$(MAKE) draft -C Synopsis
	$(MAKE) draft -C Dissertation

clean:
	#	$(MAKE) clean -C Dissertation
	latexmk -C dissertation
	rm -f dissertation.bbl
	#	$(MAKE) clean -C Synopsis
	latexmk -C synopsis
	rm -f synopsis.bbl

distclean:
	$(MAKE) distclean -C Dissertation
	$(MAKE) distclean -C Synopsis
	## Core latex/pdflatex auxiliary files:
	rm -f *.aux
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.fls
	rm -f *.out
	rm -f *.toc

	## Intermediate documents:
	rm -f *.dvi
	rm -f *-converted-to.*
	# these rules might exclude image files for figures etc.
	# *.ps
	# *.eps
	# *.pdf

	## Bibliography auxiliary files (bibtex/biblatex/biber):
	rm -f *.bbl
	rm -f *.bcf
	rm -f *.blg
	rm -f *-blx.aux
	rm -f *-blx.bib
	rm -f *.brf
	rm -f *.run.xml

	## Build tool auxiliary files:
	rm -f *.fdb_latexmk
	rm -f *.synctex
	rm -f *.synctex.gz
	rm -f *.synctex.gz\(busy\)
	rm -f *.pdfsync

	## Auxiliary and intermediate files from other packages:

	# algorithms
	rm -f *.alg
	rm -f *.loa

	# achemso
	rm -f acs-*.bib

	# amsthm
	rm -f *.thm

	# beamer
	rm -f *.nav
	rm -f *.snm
	rm -f *.vrb

	#(e)ledmac/(e)ledpar
	rm -f *.end
	rm -f *.[1-9]
	rm -f *.[1-9][0-9]
	rm -f *.[1-9][0-9][0-9]
	rm -f *.[1-9]R
	rm -f *.[1-9][0-9]R
	rm -f *.[1-9][0-9][0-9]R
	rm -f *.eledsec[1-9]
	rm -f *.eledsec[1-9]R
	rm -f *.eledsec[1-9][0-9]
	rm -f *.eledsec[1-9][0-9]R
	rm -f *.eledsec[1-9][0-9][0-9]
	rm -f *.eledsec[1-9][0-9][0-9]R

	# glossaries
	rm -f *.acn
	rm -f *.acr
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls

	# gnuplottex
	rm -f *-gnuplottex-*

	# hyperref
	rm -f *.brf

	# knitr
	rm -f *-concordance.tex
	rm -f *.tikz
	rm -f *-tikzDictionary

	# listings
	rm -f *.lol

	# makeidx
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist

	# minitoc
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc[0-9]
	rm -f *.mtc[1-9][0-9]

	# minted
	rm -f _minted*
	rm -f *.pyg

	# morewrites
	rm -f *.mw

	# mylatexformat
	rm -f *.fmt

	# nomencl
	rm -f *.nlo

	# sagetex
	rm -f *.sagetex.sage
	rm -f *.sagetex.py
	rm -f *.sagetex.scmd

	# sympy
	rm -f *.sout
	rm -f *.sympy
	rm -f sympy-plots-for-*.tex/

	# pdfcomment
	rm -f *.upa
	rm -f *.upb

	#pythontex
	rm -f *.pytxcode
	rm -f pythontex-files-*/

	# Texpad
	rm -f .texpadtmp

	# TikZ & PGF
	rm -f *.dpth
	rm -f *.md5
	rm -f *.auxlock

	# todonotes
	rm -f *.tdo

	# xindy
	rm -f *.xdy

	# WinEdt
	rm -f *.bak
	rm -f *.sav

	# endfloat
	rm -f *.ttt
	rm -f *.fff
	rm -f *.aux
	rm -f *.bbl
	rm -f *.blg
	rm -f *.dvi
	rm -f *.fdb_latexmk
	rm -f *.fls
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.nav
	rm -f *.nlo
	rm -f *.out
	rm -f *.pdfsync
	rm -f *.ps
	rm -f *.snm
	rm -f *.synctex.gz
	rm -f *.toc
	rm -f *.vrb
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc0
	rm -f *.bak
	rm -f *.bcf
	rm -f *.run.xml

release: all
	git add dissertation.pdf
	git add synopsis.pdf


==> PSCyr/pscyr/doc/PROBLEMS <==
This file explains how to solve some known problems occuring in PSCyr-0.4.

Q. dvips produces an error message "First number not found. ERROR in
   encoding vector in <...>".
A. Your dvips file is old.  Either upgrade to newer dvips (version 5.86
   or higher) or use your dvips with the -j0 option.

Q. Acrobat 4 issues the message "CRBUTR+AntiquaPSCyr-Bold contains a bad
   /BBox".
A. You have an old version of pdftex.  Upgrade to a newer one (current
   stable version is 0.14f).

Q. Acrobat 4 doesn't show the CourierPSMT-Italic font in PDF files
   produced by pdflatex.
A. Upgrade the fonts to PSCyr-0.4b or prepare your PDF file from PostScript
   using gs6** (tex->dvi->ps->pdf).

Q. Acrobat 4 issues the message "Unable to extract the embedded font
   'AACDDA+CourierPSMT-Italic'. Some characters may not display or print
   correctly" when reading PDF files produced by pdflatex.
A. Upgrade the fonts to PSCyr-0.4b or prepare your PDF file from PostScript
   using gs6** (tex->dvi->ps->pdf).

Q. TeX issues a warning like "Font shape `OMS/faq/m/n` undefined ..."
A. Ignore this message.  PSCyr font collection doesn't contain math and
   symbol characters that enter OMS, OML, OMX, and TS1 encoding tables.
   The required characters are taken from other fonts (like Computer Modern).

Q. TeX produces a wrong position of the ring in \AA symbol in all Russian
   fonts.
A. Comment the command "\DeclareTextCompositeCommand ..." in t2aenc.def file.


==> PSCyr/pscyr/doc/old/README.30 <==
NAME

    PSCYR package, version 0.3 from  September 10, 1998. 

DESCRIPTION 
   
    Collection of files providing support for Cyrillic 
    PostScript Fonts in LaTeX documents. 

    Final output is PostScript or PDF. 

DISTRIBUTION 

The distribution is split into two parts.

  * The first part (PsCyr-type1-03.tar.gz) 
    contains the files that are unlikely to change in 
    future releases:

    - font sources in Type 1 format;
    - Adobe font metrics.

    Fonts: Academy, Advertisement, Antiqua, College, Handbook,
       Lazurski, Magazine, Textbook, ArialCyrMT, CourierCyrPS,
       ERKurierKOI8RRegular, TimesNRCyrMT.

  * The second part (PsCyr-tex-03.tar.gz) 
    contains the files that are liable to modifications:
   
    - installation instructions (this file);
    - TeX font metrics;
    - font definitions; 
    - encodings; 
    - font mappings for DVIPS and pdfTeX
    - style and examples of usage;
    - scripts for generation of TeX font metrics and the map
      file.


INSTALLATION

  * Requirements

    - T2 package for LaTeX. This package is available from  
      CTAN:macros/latex/contrib/supported/t2. 
      It provides support for T2* Cyrillic TeX encodings. 
    - Dvips or pdf-LaTeX installed. Ghostscript (ghostview) or
      Acrobat Reader to visualize and print PostScript/PDF
      documents.


  * Procedure

     - Unpack the distribution: PsCyr-type1-[version].tar.gz,
                                PsCyr-tex-[version].tar.gz.

    TeX:
 
    - Copy the .tfm and .fd files to where TeX can find them.
    - Modify if necessary the TFMFONTS and TEXINPUTS environment
      variables.


    DVIPS:

    - Copy the .pfb and .enc files to where DVIPS headers reside.
    - Modify if necessary the DVIPSHEADERS environment variable. 
    - Add the string
         p +pscyr.map
      to the global configuration file config.ps, or
      to .dvipsrc in your home directory (UNIX).
    - Specify the path to pscyr.map in the TEXCONFIG environment
      variable.


    pdfTeX:
  
    - Copy the .pfb, .enc, and pscyr.map files to where pdfTeX
      headers reside.
    - Add the string
         map +pscyr.map
      to the global configuration file pdftex.cfg.
    - If you don't have permission to modify the global
      pdftex.cfg (UNIX), modify local copy and specify its 
      location in the TEXPSHEADERS environment variable.



USAGE 

  * LaTeX

Once the installation is made for LaTeX, Cyrillic PostScript
fonts become available in LaTeX documents. For example,
   
   \usefont{T2A}{faq}{m}{n} 

loads the Antiqua font at medium weight and upright shape.  You
may redefine the default font family by issuing the command

   \renewcommand{\rmdefault}{faq} 

in the header. See the examples provided and the style file
pscyr.sty. Also look at the font definitions for available
weights and shapes for different font families.


  * Printing and previewing

After the document is converted to PostScript by DVIPS, it can be
visualized and printed with ghostscript/ghostview.

++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
ATTENTION: Use DVIPS with -j0 option. Otherwise font re-encoding
           does not work properly.
++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

pdfLaTeX creates PDF directly from TeX source. This can be
printed and previewed with freely available Acrobat Reader.


  * Adding new fonts (UNIX only) 

You may use the perl scripts located in ./src to generate TeX
font metrics and the map file. These scripts are batch files for
afm2tfm program, which must be installed on your system. The
procedure is the following.

    - Copy Adobe font metrics of the new font to ./afm
   
    - Choose or create the appropriate encoding vector in ./enc.
    - Modify the file fontmap.txt in ./src. The syntax is

      TFM_NAME TMP_NAME AFM_NAME EFFECTS

      TFM_NAME : name of TeX font metrics file to create;
      TMP_NAME : unique name of temporary tfm file, which will be
                 created and erased by the script;
      AFM_NAME : name of Adobe font metrics file;

      EFFECTS  : E -extended, e - condensed, s - slanted. 
                 [012] - number of .enc file containing
                 the encoding vector.

    - Run the script make-all.sh. The .tfm and .map files will be
      created.

NOTES

The PSCYR package is unsupported, though serious bugs get fixed
somehow. The most serious problem is the quality of free fonts
included in the distribution: non-standard encodings, absent
ligatures, no kerning.

The typefaces included in this package originally come from   

    - The Monotype Corporation plc. (with changes by 
      Eugene V. Demidov);
    - Gavin Helf (with changes by Andrey A. Chernov);
    - ParaType, division of ParaGraph International.  

As to my knowledge, these fonts are placed into public domain and
can be freely redistributed.

COPYRIGHT 

The PSCYR package is free software provided "as is" without any
warranty.  You can redistribute it and/or modify it, provided
that the same notice appears in the modified version.


AUTHOR

Konstantin Chumachenko <chumachenko@writeme.com>;

thanks to:

Vladimir Volovich <TeX@vvv.vsu.ru>, for scripts and bug fixes;
Vitaly Repin <2:5030/209.26@fidonet.org>, for PSCYR style file. 
    


==> Synopsis/Makefile <==
all:
	latexmk -pdf -pdflatex="xelatex %O %S" synopsis

pdf:
	latexmk -pdf -jobname=synopsis_pdf -silent  synopsis.tex
# xedraft:
# 	xelatex -ini "&pdflatex draft-preamble.tex\dump"
# 	latexmk -pdf -pdflatex="xelatex %O %S" draft
draft:
	pdflatex -ini -jobname="draft-preamble" "&pdflatex draft-preamble.tex\dump"
	latexmk -pdf -jobname=draft -silent --shell-escape draft.tex

clean:
	latexmk -C synopsis
	rm -f synopsis.bbl

distclean:
	## Core latex/pdflatex auxiliary files:
	rm -f *.aux
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.fls
	rm -f *.out
	rm -f *.toc

	## Intermediate documents:
	rm -f *.dvi
	rm -f *-converted-to.*
	# these rules might exclude image files for figures etc.
	# *.ps
	# *.eps
	# *.pdf

	## Bibliography auxiliary files (bibtex/biblatex/biber):
	rm -f *.bbl
	rm -f *.bcf
	rm -f *.blg
	rm -f *-blx.aux
	rm -f *-blx.bib
	rm -f *.brf
	rm -f *.run.xml

	## Build tool auxiliary files:
	rm -f *.fdb_latexmk
	rm -f *.synctex
	rm -f *.synctex.gz
	rm -f *.synctex.gz\(busy\)
	rm -f *.pdfsync

	## Auxiliary and intermediate files from other packages:

	# algorithms
	rm -f *.alg
	rm -f *.loa

	# achemso
	rm -f acs-*.bib

	# amsthm
	rm -f *.thm

	# beamer
	rm -f *.nav
	rm -f *.snm
	rm -f *.vrb

	#(e)ledmac/(e)ledpar
	rm -f *.end
	rm -f *.[1-9]
	rm -f *.[1-9][0-9]
	rm -f *.[1-9][0-9][0-9]
	rm -f *.[1-9]R
	rm -f *.[1-9][0-9]R
	rm -f *.[1-9][0-9][0-9]R
	rm -f *.eledsec[1-9]
	rm -f *.eledsec[1-9]R
	rm -f *.eledsec[1-9][0-9]
	rm -f *.eledsec[1-9][0-9]R
	rm -f *.eledsec[1-9][0-9][0-9]
	rm -f *.eledsec[1-9][0-9][0-9]R

	# glossaries
	rm -f *.acn
	rm -f *.acr
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls

	# gnuplottex
	rm -f *-gnuplottex-*

	# hyperref
	rm -f *.brf

	# knitr
	rm -f *-concordance.tex
	rm -f *.tikz
	rm -f *-tikzDictionary

	# listings
	rm -f *.lol

	# makeidx
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist

	# minitoc
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc[0-9]
	rm -f *.mtc[1-9][0-9]

	# minted
	rm -f _minted*
	rm -f *.pyg

	# morewrites
	rm -f *.mw

	# mylatexformat
	rm -f *.fmt

	# nomencl
	rm -f *.nlo

	# sagetex
	rm -f *.sagetex.sage
	rm -f *.sagetex.py
	rm -f *.sagetex.scmd

	# sympy
	rm -f *.sout
	rm -f *.sympy
	rm -f sympy-plots-for-*.tex/

	# pdfcomment
	rm -f *.upa
	rm -f *.upb

	#pythontex
	rm -f *.pytxcode
	rm -f pythontex-files-*/

	# Texpad
	rm -f .texpadtmp

	# TikZ & PGF
	rm -f *.dpth
	rm -f *.md5
	rm -f *.auxlock

	# todonotes
	rm -f *.tdo

	# xindy
	rm -f *.xdy

	# WinEdt
	rm -f *.bak
	rm -f *.sav

	# endfloat
	rm -f *.ttt
	rm -f *.fff
	rm -f *.aux
	rm -f *.bbl
	rm -f *.blg
	rm -f *.dvi
	rm -f *.fdb_latexmk
	rm -f *.fls
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.nav
	rm -f *.nlo
	rm -f *.out
	rm -f *.pdfsync
	rm -f *.ps
	rm -f *.snm
	rm -f *.synctex.gz
	rm -f *.toc
	rm -f *.vrb
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc0
	rm -f *.bak
	rm -f *.bcf
	rm -f *.run.xml


==> Synopsis/content.tex <==
\subsection*{Общая характеристика работы}

\newcommand{\actuality}{\underline{\textbf{Актуальность темы.}}}
\newcommand{\aim}{\underline{\textbf{Целью}}}
\newcommand{\tasks}{\underline{\textbf{задачи}}}
\newcommand{\defpositions}{\underline{\textbf{Основные положения, выносимые на~защиту:}}}
\newcommand{\novelty}{\underline{\textbf{Научная новизна:}}}
\newcommand{\influence}{\underline{\textbf{Практическая значимость}}}
\newcommand{\reliability}{\underline{\textbf{Достоверность}}}
\newcommand{\probation}{\underline{\textbf{Апробация работы.}}}
\newcommand{\contribution}{\underline{\textbf{Личный вклад.}}}
\newcommand{\publications}{\underline{\textbf{Публикации.}}}

\input{common/characteristic} % Характеристика работы по структуре во введении и в автореферате не отличается (ГОСТ Р 7.0.11, пункты 5.3.1 и 9.2.1), потому её загружаем из одного и того же внешнего файла, предварительно задав форму выделения некоторым параметрам

%Диссертационная работа была выполнена при поддержке грантов ...

%\underline{\textbf{Объем и структура работы.}} Диссертация состоит из~введения, четырех глав, заключения и~приложения. Полный объем диссертации \textbf{ХХХ}~страниц текста с~\textbf{ХХ}~рисунками и~5~таблицами. Список литературы содержит \textbf{ХХX}~наименование.

%\newpage
\subsection*{Содержание работы}
Во \underline{\textbf{введении}} обосновывается актуальность исследований, проводимых в рамках данной диссертационной работы, приводится обзор научной литературы по изучаемой проблеме, формулируется цель, ставятся задачи работы, сформулированы научная новизна и практическая значимость представляемой работы.

\underline{\textbf{Первая глава}} посвящена ...

 картинку можно добавить так:
\begin{figure}[ht] 
  \center
  \includegraphics [scale=0.27] {latex}
  \caption{Подпись к картинке.} 
  \label{img:latex}
\end{figure}

Формулы в строку без номера добавляются так:
\[ 
  \lambda_{T_s} = K_x\frac{d{x}}{d{T_s}}, \qquad
  \lambda_{q_s} = K_x\frac{d{x}}{d{q_s}},
\]

\underline{\textbf{Вторая глава}} посвящена исследованию 

\underline{\textbf{Третья глава}} посвящена исследованию 

В \underline{\textbf{четвертой главе}} приведено описание 

В \underline{\textbf{заключении}} приведены основные результаты работы, которые заключаются в следующем:
\input{common/concl}


%\newpage
При использовании пакета \verb!biblatex! список публикаций автора по теме
диссертации формируется в разделе <<\publications>>\ файла
\verb!../common/characteristic.tex!  при помощи команды \verb!\nocite! 

\ifthenelse{\equal{\thebibliosel}{0}}{% Встроенная реализация с загрузкой файла через движок bibtex8
  \renewcommand{\refname}{\large \authorbibtitle}
  \nocite{*}
  \insertbiblioauthor                          % Подключаем Bib-базы
  %\insertbiblioother   % !!! bibtex не умеет работать с несколькими библиографиями !!!
}{% Реализация пакетом biblatex через движок biber
  \insertbiblioauthor                          % Подключаем Bib-базы
  \insertbiblioother
}



==> Synopsis/draft.tex <==
%&draft-preamble
\begin{document}

\input{title}           % Титульный лист
\subimport{../}{content}         % Содержание автореферата

\end{document}

==> Synopsis/setup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Файл упрощённых настроек шаблона диссертации %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%        Подключение пакетов                 %%%
\usepackage{ifthen}                 % добавляет ifthenelse
%%% Инициализирование переменных, не трогать!  %%%
\newcounter{bibliosel}
\newcounter{tabcap}
\newcounter{tablaba}
\newcounter{tabtita}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Область упрощённого управления оформлением %%%

%% Библиография

%% Внимание! При использовании bibtex8 необходимо удалить все
%% цитирования из  ../common/characteristic.tex 
\setcounter{bibliosel}{1}           % 0 --- встроенная реализация с загрузкой файла через движок bibtex8; 1 --- реализация пакетом biblatex через движок biber

%% Подпись таблиц
\setcounter{tabcap}{0}              % 0 --- по ГОСТ, номер таблицы и название разделены тире, выровнены по левому краю, при необходимости на нескольких строках; 1 --- подпись таблицы не по ГОСТ, на двух и более строках, дальнейшие настройки: 
%Выравнивание первой строки, с подписью и номером
\setcounter{tablaba}{2}             % 0 --- по левому краю; 1 --- по центру; 2 --- по правому краю
%Выравнивание строк с самим названием таблицы
\setcounter{tabtita}{1}             % 0 --- по левому краю; 1 --- по центру; 2 --- по правому краю

%%% Цвета гиперссылок %%%
% Latex color definitions: http://latexcolor.com/
\definecolor{linkcolor}{rgb}{0.9,0,0}
\definecolor{citecolor}{rgb}{0,0.6,0}
\definecolor{urlcolor}{rgb}{0,0,1}
%\definecolor{linkcolor}{rgb}{0,0,0} %black
%\definecolor{citecolor}{rgb}{0,0,0} %black
%\definecolor{urlcolor}{rgb}{0,0,0} %black

==> Synopsis/synpackages.tex <==
%%% Опционально %%%
% Следующий пакет может быть полезен, если надо ужать текст, чтобы сам текст не править, но чтобы места он занимал поменьше
%\usepackage{savetrees}

% Этот пакет может быть полезен для печати текста брошюрой
%\usepackage[print]{booklet}

==> Synopsis/synstyles.tex <==
%%% Изображения %%%
\graphicspath{{images/}{Synopsis/images/}}         % Пути к изображениям

%%% Макет страницы %%%
\oddsidemargin=-13pt
\topmargin=-66pt
\headheight=12pt
\headsep=38pt
\textheight=732pt
\textwidth=484pt
\marginparsep=14pt
\marginparwidth=43pt
\footskip=14pt
\marginparpush=7pt
\hoffset=0pt
\voffset=0pt
%\paperwidth=597pt
%\paperheight=845pt
\parindent=1.5cm                  % Размер табуляции (для красной строки) в начале каждого абзаца
\renewcommand{\baselinestretch}{1.25}

\newcommand{\sfs}{\fontsize{14pt}{15pt}\selectfont}
\sfs % размер шрифта и расстояния между строками


==> Synopsis/title.tex <==
\thispagestyle{empty}

\vspace{0pt plus1fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{flushright}
  \large{На правах рукописи}
  \includegraphics[height=1.5cm]{personal-signature} 
\end{flushright}

\vspace{0pt plus3fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}
\textbf {\large \thesisAuthor}
\end{center}

\vspace{0pt plus3fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}
\textbf {\Large \thesisTitle}

\vspace{0pt plus3fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
{\large Специальность \thesisSpecialtyNumber\ "---\par <<\thesisSpecialtyTitle>>}

\vspace{0pt plus1.5fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\Large{Автореферат}\par
\large{диссертации на соискание учёной степени\par \thesisDegree}
\end{center}

\vspace{0pt plus4fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}
{\large{\thesisCity\ "--- \thesisYear}}
\end{center}

\newpage
% оборотная сторона обложки
\thispagestyle{empty}
\noindent Работа выполнена в \thesisInOrganization

\par\bigskip
%\begin{table}[h] % считается не очень правильным использовать окружение table, не задавая caption
    \noindent%
    \begin{tabular}{@{}lp{11cm}}
        \sfs Научный руководитель: & \sfs \supervisorRegalia \par
                                      \textbf{\supervisorFio}
        \vspace{4mm} \\
        {\sfs Официальные оппоненты:} &
        {\sfs \textbf{\opponentOneFio,}\par
                  \opponentOneRegalia,\par
                  \opponentOneJobPlace,\par
                  \opponentOneJobPost\par \vspace{3mm}
                  \textbf{\opponentTwoFio,}\par \vspace{1mm}
                  \opponentTwoRegalia,\par
                  \opponentTwoJobPlace,\par
                  \opponentTwoJobPost
        }
        \vspace{4mm} \\
        {\sfs Ведущая организация:} & {\sfs \leadingOrganizationTitle }
    \end{tabular}  
%\end{table}
\par\bigskip

\noindent Защита состоится \defenseDate~на~заседании диссертационного совета \defenseCouncilNumber~на базе \defenseCouncilTitle~по адресу: \defenseCouncilAddress.

\vspace{5mm}
\noindent С диссертацией можно ознакомиться в библиотеке \synopsisLibrary.

\vspace{5mm}
\noindent{Автореферат разослан \synopsisDate.}

\vspace{5mm}
%\begin{table} [h] % считается не очень правильным использовать окружение table, не задавая caption
\par\bigskip
    \noindent%
    \begin{tabular}{p{8cm}cr}
        \begin{tabular}{p{8cm}}
            \sfs Ученый секретарь  \\
            \sfs диссертационного совета  \\
            \sfs \defenseCouncilNumber, \defenseSecretaryRegalia
        \end{tabular} 
    &
        \begin{tabular}{c}
            \includegraphics[height=1cm]{secretary-signature} 
        \end{tabular} 
    &
        \begin{tabular}{r}
            \\
            \\
            \sfs \defenseSecretaryFio
        \end{tabular} 
    \end{tabular}
%\end{table}
\newpage


==> common/concl.tex <==
%% Согласно ГОСТ Р 7.0.11-2011:
%% 5.3.3 В заключении диссертации излагают итоги выполненного исследования, рекомендации, перспективы дальнейшей разработки темы.
%% 9.2.3 В заключении автореферата диссертации излагают итоги данного исследования, рекомендации и перспективы дальнейшей разработки темы.
\begin{enumerate}
  \item На основе анализа \ldots
  \item Численные исследования показали, что \ldots
  \item Математическое моделирование показало \ldots
  \item Для выполнения поставленных задач был создан \ldots
\end{enumerate}

